Teaching Higher-Order Logic Using Isabelle

We present a formalization of higher-order logic in the Isabelle proof assistant, building directly on the foundational framework Isabelle/Pure and developed to be as small and readable as possible. It should therefore serve as a good introduction for someone looking into learning about higher-order logic and proof assistants, without having to study the much more complex Isabelle/HOL with heavier automation. To showcase our development and approach we explain a sample proof, describe the axioms and rules of our higher-order logic, and discuss our experience with teaching the subject in a classroom setting.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{J. Narboux, W. Neuper and P. Quaresma (Eds.): Workshop on\\ Theorem proving components for Educational software 2023 (ThEdu'23)\\
EPTCS 400, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.400.5}{10.4204/EPTCS.400.5}}
\pdfoutput=1

